An end-to-end calibration of the Mini-EUSO detector in space

Mini-EUSO is a wide Field-of-View (FoV, 44$^{\circ}$) telescope currently in operation from a nadia-facing UV-transparent window in the Russian Zvezda module on the International Space Station (ISS). It is the first detector of the JEM-EUSO program deployed on the ISS, launched in August 2019. The main goal of Mini-EUSO is to measure the UV emissions from the ground and atmosphere, using an orbital platform. Mini-EUSO is mainly sensitive in the 290-430 nm bandwidth. Light is focused by a system of two Fresnel lenses of 25 cm diameter each on the Photo- Detector-Module (PDM), which consists of an array of 36 Multi-Anode Photomultiplier Tubes (MAPMTs), for a total of 2304 pixels working in photon counting mode, in three different time resolutions of 2.5 ${\mu}$s, 320 ${\mu}$s, 40.96 ms operation in parallel. In the longest time scale, the data is continuously acquired to monitor the UV emission of the Earth. It is best suited for the observation of ground sources and therefore has been used for the observational campaigns of the Mini-EUSO. In this contribution, we present the assembled UV flasher, the operation of the field campaign and the analysis of the obtained data. The result is compared with the overall efficiency computed from the expectations which takes into account the atmospheric attenuation and the parameterization of different effects such as the optics efficiency, the MAPMT detection efficiency, BG3 filter transmittance and the transparency of the ISS window.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

